Decremental Matching in General Weighted Graphs

In this paper, we consider the problem of maintaining a $(1-\varepsilon)$-approximate maximum weight matching in a dynamic graph $G$, while the adversary makes changes to the edges of the graph. In the fully dynamic setting, where both edge insertions and deletions are allowed, Gupta and Peng gave an algorithm for this problem with an update time of $\tilde{O}_{\varepsilon}(\sqrt{m})$. We study a natural relaxation of this problem, namely the decremental model, where the adversary is only allowed to delete edges. For the cardinality version of this problem in general (possibly, non-bipartite) graphs, Assadi, Bernstein, and Dudeja gave a decremental algorithm with update time $O_{\varepsilon}(\text{poly}(\log n))$. However, beating $\tilde{O}_{\varepsilon}(\sqrt{m})$ update time remained an open problem for the \emph{weighted} version in \emph{general graphs}. In this paper, we bridge the gap between unweighted and weighted general graphs for the decremental setting. We give a $O_{\varepsilon}(\text{poly}(\log n))$ update time algorithm that maintains a $(1-\varepsilon)$-approximate maximum weight matching under adversarial deletions. Like the decremental algorithm of Assadi, Bernstein, and Dudeja, our algorithm is randomized, but works against an adaptive adversary. It also matches the time bound for the cardinality version upto dependencies on $\varepsilon$ and a $\log R$ factor, where $R$ is the ratio between the maximum and minimum edge weight in $G$.

==> WeightMorEimp.tex <==
\subsection{Algorithm for \textsc{Weighted-Frac-Match}()}

The final ingredient we need for \textsc{WeightedM-or-E*}() is the following lemma, which computes a fractional matching on low capacity edges.

\begin{lemma2}\label{lem:Hungarian2}
Consider a weighted bipartite multi-graph $G$ with edge capacity function $\kappa$, and edge weights in $\set{1,2,\cdots, W}$. There is an algorithm that in $O(m\cdot W\cdot \log n\cdot \nicefrac{1}{\eps})$ time finds a fractional matching $\vec{x}$ obeting the capacity function $\kappa$ such that $\sum_{e\in E}w(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G,\kappa)$.
\end{lemma2}

In order to come up with this algorithm, we first recall the maximum weight capacitated fractional matching linear program for bipartite graphs, and its corresponding dual.

\begin{equation}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{e\in E} w(e)\cdot x(e)  \\
\text{subject to}& \displaystyle x(e)\leqslant \kappa(e)& & \forall e\in E \\
& \displaystyle \sum_{e\ni v} x(e) \leqslant 1 & & \forall v\in V
\end{array}
\end{equation}

\begin{equation}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle\sum\limits_{v\in L} y(v) +\sum\limits_{u\in R} y(u) +\sum_{e\in E} z(e)\cdot \kappa(e) &  \\
\text{subject to}& \displaystyle yz(e)\geqslant w(e) &  \forall e\in E 
\end{array}
\end{equation}

Here, $yz(e)=y(u)+y(v)+z(e)$, where $u,v$ are the two endpoints of $e$. Additionally, before stating our algorithm, we give some definitions.

\begin{definition2}[Residual Graph]
Given a bipartite graph $G=(L,R,E)$, with a capacity function $\kappa$ on the edges of the graph. Let $\vec{x}$ be a fractional matching obeying $\kappa$. We define $G_x$ to be the residual graph with respect to $\vec{x}$. In particular, this is a directed graph, where corresponding to each undirected edge $e\in G$, there are two directed edges, $e_f$ (forward edges, directed from $L$ to $R$), and $e_b$ (backward edge, directed from $R$ to $L$). Moreover, $e_f$ has a residual capacity of $\kappa(e)-x(e)$, and $e_b$ has a capacity of $x(e)$. 
\end{definition2}

\begin{definition2}[Free Vertices]
Given a graph $G$, and a fractional matching $\vec{x}$, we say that a vertex $v$ is free with respect to $\vec{x}$ if $\sum_{e\ni v}x(e)<1$.
\end{definition2}

\begin{definition2}
    An augmenting path in $G_x$, will refer to a path starting and ending in a free a vertex, and all the intermediate vertices on this path will be saturated.
\end{definition2}

Before stating our algorithm, we will state the invariants that the algorithm will maintain. Subsequently, we will show that maintaining these invariants throughout implies that the algorithm will output a matching satisfying the approximation guarantees of \Cref{lem:Hungarian2} and in the desired runtime.

\begin{proposition}\label{prop:invariants}
There is an algorithm will maintain at all times, a fractional matching $\vec{x}$, and the dual variables $y(u)$ for all $u\in V$, and $z(e)$, for all $e\in E$ with the following properties.
\begin{enumerate}
    \item \textbf{Granularity:} Throughout the algorithm, the duals $y(u)$ for all $u\in V$, and $z(e)$ for all $e\in E$, are multiples of $\eps$. \label{item:gran}
    \item \textbf{Domination:} For all directed edges $e_f$ and $e_b$ in $G_{x}$, we have $yz(e_f)\geqslant w(e)-\eps$, and $yz(e_b)\geqslant w(e)-\eps$.\label{item:domin}
    \item \textbf{Tightness:} For all backward edges $e_b$, we additionally have the property that $yz(e_b)\leqslant w(e_b)+\eps$. \label{item:tightness}
    \item \textbf{Free Duals:} The duals for free vertices $u\in L$ are equal, and are at most the dual values for other vertices. The free vertex duals in $R$ are always $0$. The algorithm terminates when the free vertex duals in $L$ are all $0$. \label{item:freeduals}
    \item \textbf{Complementary Slackness:} If $z(e)>0$ for some $e\in E$, then $x(e)=\kappa(e)$. \label{item:slackness}
\end{enumerate}
\end{proposition}

\begin{definition2}[Eligible Edges]
    Let $\vec{x}$ be the current fractional matching maintained by the graph, and let $G_{x}$ denote the residual graph with respect to $\vec{x}$. A forward edge $e_f$ is eligible if $yz(e_f) = w(e)-\eps$, and backward edge $e_b$ is said to be eligible if $yz(e_b)=w(e)+\eps$. We use $G^t_x$ to denote the eligible subgraph of $G_x$. 
\end{definition2}

\begin{lemma2}
The fractional matching $\vec{x}$ returned by the algorithm mentioned in \Cref{prop:invariants} has $\sum_{e\in E}w(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)$.
\end{lemma2}

\begin{proof}
    In order to see this, consider the dual variables returned by the algorithm. Note that if we increase each of the duals by a factor of $(1+\eps)$, then the dual solutions $\vec{y},\vec{z}$ maintained by the algorithm are feasible dual solutions to the dual program. Thus, by weak duality, we have,
    \begin{align*}
        \sum_{u\in V}y(u)+\sum_{e\in E} z(e)\cdot \kappa(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)
    \end{align*}
    Due to complementary slackness, (\Cref{prop:invariants}\ref{item:slackness}
    ), we have,
    \begin{align*}
        \sum_{u\in V} y(u) +\sum_{e\in E} x(e)\cdot z(e) \geqslant (1-\eps)\cdot \textsf{mwm}(G)
    \end{align*}
\end{proof}

We now want to state the precise algorithm.
\begin{algorithm}[H] 
	\algorithmicrequire{ A bipartite multigraph $G$ with capacity and weight edge functions $\kappa$ and $w$.}\\
	\algorithmicensure{ A fractional matching $\vec{x}$ with $\sum_{e\in E}w(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G,\kappa)$}
	\caption{\textsc{Weighted-Frac-Matching}($G,\kappa,\eps$)}
	\begin{algorithmic}[1]
	\Procedure{Initialization:}{}
		\State $x(e)\leftarrow 0$ for all $e\in E$ \Comment{Initializing $\vec{x}$}
		\State $y(u)\leftarrow W-\eps\cdot W$ for all $u\in L$ \Comment{Initializing left vertex duals.}
		\State $y(u)\leftarrow 0$ for all $u\in R$ \Comment{Initializing right vertex duals.}
		\State $z(e)\leftarrow 0$ for all $e\in E$ \Comment{Initializing edge duals.}
	\EndProcedure
	\State Execute scales $i=1,\cdots, \log W$ and return fractional matching $\vec{x}$.
	\State \textbf{Scale $i$}:
		\While{$y$-values of free left vertices are greater than $\frac{W-\eps\cdot W}{2^i}$}
		\For{$e_b\in G^t_x$ with $z(e)>0$}
		\State $z(e)\leftarrow z(e)-\min\set{z(e), yz(e)-w_i(e)+\delta_i}$. \Comment{Either $z(e)=0$, or $e\notin G^t_x$ as $yz(e)=w_{i}(e)-\delta_i$} \label{item:zadj} 
		\EndFor
		\State Update $G^t_x$
		\Procedure{Augmentation:}{} 
		\State Find the maximal set $\mathcal{P}$ of augmenting paths in $G^t_x$. \label{item:augpath}
		\State Augment along $\mathcal{P}$.  \label{item:augmentation}
		\State Update $\vec{x}$ and $G^t_x$.  \label{item:augmentation2}
		\EndProcedure
	\Procedure{Dual Adjustment:}{}
		\State Let $Z$ be the set of vertices reachable from free left vertices in $G^t_x$.
		\State For all ineligible edges $e_b$ directed from $R\setminus Z$ to $L\cap Z$, $z(e)\leftarrow z(e)+\delta_i$.
		\State For all $u\in L\cap Z$, $y(u)\leftarrow y(u)-\delta_i$.
		\State For all $u\in R\cap Z$, $y(u)\leftarrow y(u)+\delta_i$.
	\EndProcedure
		\EndWhile
	\Procedure{Prepare for next scale:}{}
		\State $\delta_{i+1}\leftarrow \frac{\delta_{i}}{2}$
		\State $y(u)\leftarrow y(u)+2\delta_{i+1}$ for all $u\in L$
	\EndProcedure
		\end{algorithmic}
	 \label{alg:weightedfracmatching}
\end{algorithm}

==> WeightedM-orE.tex <==
 \subsection{Algorithm for \textsc{Weighted-Frac-Match}()}

The final ingredient we need for \textsc{WeightedM-or-E*}(), is the following lemma, which computes a fractional matching on low capacity edges.

\begin{lemma2}
Consider a weighted bipartite graph $G$ with edge capacity function $\kappa$, and edge weights in $\set{1,2,\cdots,W}$. There is an algorithm that in $O(\nicefrac{m}{\eps}\cdot \log \nicefrac{1}{\eps})$ time finds a fractional matching $\vec{x}$ obeying the capacity function $\kappa$ such that $\sum_{e\in E}w(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G,\kappa)$. 
\end{lemma2}

In order to come up with this algorithm, first recall the maximum weight capacitated fractional matching linear program, and its corresponding dual.

\begin{equation}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{e\in E} w(e)\cdot x(e)  \\
\text{subject to}& \displaystyle x(e)\leqslant \kappa(e)& & \forall e\in E \\
& \displaystyle \sum_{e\ni v} x(e) \leqslant 1 & & \forall v\in V
\end{array}
\end{equation}

\begin{equation}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle\sum\limits_{v\in L} y(v) +\sum\limits_{u\in R} y(u) +\sum_{e\in E} z(e)\cdot \kappa(e) &  \\
\text{subject to}& \displaystyle yz(e)\geqslant w(e) &  \forall e\in E 
\end{array}
\end{equation}

Here, $yz(e)=y(u)+y(v)+z(e)$, where $u,v$ are the two endpoints of $e$. We will come up with an algorithm that maintains the following invariants at all times. We denote $\delta_0=\eps\cdot W$, and $\delta_{i}=\nicefrac{\delta_0}{2^i}$. Additionally, for an edge $e$, we denote by $w_i(e)=\left\lfloor \frac{w(e)}{\delta_i}\right \rfloor\cdot \delta_i$, the truncated weight function at scale $i$. We additionally assume that $W$ and $\eps$ are powers of $2$. 

\begin{definition2}
Given a bipartite graph $G$, with a capacity function $\kappa$ on the edges of the graph. Suppose $\vec{x}$ is a fractional matching on edges of the graph, obeying the capacity function $\kappa$. We define $G_x$ to be the residual graph with respect to $\vec{s}$. This is a directed graph, where, corresponding to every edge $e$, there is a forward edge $e_f$, and a backward edge $e_b$, and capacity of $e_f$ is $\kappa(e)-x(e)$, and $e_b$ has capacity $x(e)$. 
\end{definition2}

 We additionally define free vertices as follows:

\begin{definition2}
Given a graph $G$ and a fractional matching $\vec{x}$, we say that a vertex $v$ is free with respect to $\vec{x}$ if $\sum_{e\ni v}x(e)<1$.
\end{definition2}

\begin{property}\label{prop:invariant} The algorithm will maintain at all times, a fractional matching $\vec{x}$, and dual variables $y(u)$ for all $u\in V$, and $z_e$ for all $e\in E$. The algorithm will proceed in $i=1,2,\cdots, \log W$ scales, and in each scale $i$, we will maintain the following properties in the residual graph $G_x$. 
\begin{enumerate}
\item \textbf{Granularity:} The dual variable $y(u)$ is a multiple of $\delta_i$, and similarly, $z(e)$ is a multiple of $\delta_i$. \label{item:gran}
\item \textbf{Near Domination:} For all edges $e_f$ and $e_b$, we have $yz(e_f)\geqslant w_i(e)-\delta_i$, and $yz(e_b)\geqslant w_i(e)-\delta_i$. \label{item:domin}
\item \textbf{Tightness:} For all back edges $e_b$, we have, $yz(e_b)\leqslant w_i(e)+2\cdot(\delta_j-\delta_i)$, where $j$ is the scale at which $e_b$ last existed in $G_x$ (with non-zero capacity), and was never removed. We say that in this case that $e_b$ is a backward edge of type $j$.  \label{item:tightness}
\item \textbf{Free Duals:} The duals $y(u)$ for free $u\in L$ are equal, and are at most the dual values for all other vertices. We stop scale $i$ when free vertex duals in $L$ reach value $\nicefrac{W}{2^{i+1}}-\nicefrac{\eps\cdot W}{2^{i+1}}$. On the other hand, the duals $y(u)$ for all free $u\in R$ are zero throughout the run of the algorihm. At the end of the scale $\log W$, all free vertex duals $y(u)$ are $0$.\label{item:freeduals}
\item \textbf{Complementary Slackness:} If $z(e)>0$ for some $e\in E$, then $x(e)=\kappa(e)$. \label{item:slackness}
\end{enumerate} 
\end{property}

Our goal will be to first show that if an algorithm maintains invariants mentioned in \Cref{prop:invariant}, then at the end of the algorithm, we have a matching $M$ with $w(M)\geqslant (1-\eps)\cdot \textsf{mwm}(G,\kappa)$. In order to do this, we start with some definitions.

\begin{definition2}[Eligible Edges]
Let $\vec{x}$ be the current fractional matching maintained by the graph, and let $G_x$ denote the residual graph with respect to $\vec{x}$. In scale $i$, we define a forward edge $e_f$ to be eligible if $yz(e_f)=w(e_f)-\delta_i$, and backward edge $e_b$ is eligible if $yz(e_b)-w(e_b)$ is a non-negative multiple of $\delta_i$. We use $G^t_{x}$ to denote the eligible subgraph of $G_x$. 
\end{definition2}
We first show the following intermediate claim, and thereafter, we show this claim combined with \Cref{prop:invariant}, shows that at the of the algorithm, we have $\sum_{e\in E} w(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G,\kappa)$. 

\begin{claim2}\label{claim:forward}
All eligible forward edges in scales $0$ to $i$ have weights at least $\frac{W}{2^{i+1}}$. Moreover, in scale $i$, for all backward edges of type $j$, we have $yz(e)\leqslant (1+4\eps)\cdot w(e)$.
\end{claim2}
\begin{proof}
First, consider forward edges $e_f$, these are eligible if they have the property that $yz(e)=w(e)-\delta_i$ in scale $i$. Note that the $yz(e)$ values are lower bounded by the $y(u)$ value of the free vertices which is at least $\nicefrac{W}{2^i}-\delta_i$. Therefore, it follows that $w(e)\geqslant \nicefrac{W}{2^i}$. This shows the first part of the claim. To show the second part of the claim, since $e$ is a backward edge of type $j$, this means that before scale $j$, it was solely a forward edge. Consequently, we have that $w(e)\geqslant \nicefrac{W}{2^{j+1}}$. To prove the second part of the argument, we have the following line of reasoning due \Cref{prop:invariant}\ref{item:tightness} and discussion above, 
\begin{align*}
yz(e)-w(e)&\leqslant 2(\delta_j-\delta_i)\\
&< 2\cdot \delta_j\\
&\leqslant 8\cdot\eps\cdot w(e)
\end{align*}
This proves the claim.
\end{proof}

Now, we want to a bound on the weight of the fractional matching output by the algorithm. 

\begin{claim2}
Let $\vec{x}$ be the fractional matching returned by the graph. Then, we have, $\sum_{e\in E}x(e)\cdot w(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)$.
\end{claim2}
\begin{proof}
In order to see this, consider the dual variables returned by the algorithm. We know that,
\begin{align*}
\sum_{u\in V}y(u)+\sum_{e\in E}z(e)\cdot \kappa(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)
\end{align*}
Due to complementary slackness (\Cref{prop:invariant}\ref{item:slackness}), we have,
\begin{align*}
\sum_{u\in V} y(u)+\sum_{e\in E} x(e)\cdot z(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)
\end{align*}
Due to the fact that free vertex duals, at the end of the algorithm are zero (\Cref{prop:invariant}\ref{item:freeduals}), we have,
\begin{align*}
\sum_{u\in V} \sum_{e\ni u} x(e)\cdot y(u)+\sum_{e\in E} z(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)
\end{align*}
Simplifying the above expression, we have,
\begin{align*}
\sum_{e\in E} yz(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)
\end{align*}
Using \Cref{claim:forward}, we have, 
\begin{align*}
\sum_{e\in E} (1+4\eps)\cdot w(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G)
\end{align*}
This shows the claim. 
\end{proof}
We now want to state the precise algorithm.
\begin{algorithm}[H] 
	\algorithmicrequire{ A bipartite multigraph $G$ with capacity and weight edge functions $\kappa$ and $w$.}\\
	\algorithmicensure{ A fractional matching $\vec{x}$ with $\sum_{e\in E}w(e)\cdot x(e)\geqslant (1-\eps)\cdot \textsf{mwm}(G,\kappa)$}
	\caption{\textsc{Weighted-Frac-Matching}($G,\kappa,\eps$)}
	\begin{algorithmic}[1]
	\Procedure{Initialization:}{}
		\State $x(e)\leftarrow 0$ for all $e\in E$ \Comment{Initializing $\vec{x}$}
		\State $y(u)\leftarrow W-\eps\cdot W$ for all $u\in L$ \Comment{Initializing left vertex duals.}
		\State $y(u)\leftarrow 0$ for all $u\in R$ \Comment{Initializing right vertex duals.}
		\State $z(e)\leftarrow 0$ for all $e\in E$ \Comment{Initializing edge duals.}
	\EndProcedure
	\State Execute scales $i=1,\cdots, \log W$ and return fractional matching $\vec{x}$.
	\State \textbf{Scale $i$}:
		\While{$y$-values of free left vertices are greater than $\frac{W-\eps\cdot W}{2^i}$}
		\For{$e_b\in G^t_x$ with $z(e)>0$}
		\State $z(e)\leftarrow z(e)-\min\set{z(e), yz(e)-w_i(e)+\delta_i}$. \Comment{Either $z(e)=0$, or $e\notin G^t_x$ as $yz(e)=w_{i}(e)-\delta_i$} \label{item:zadj} 
		\EndFor
		\State Update $G^t_x$
		\Procedure{Augmentation:}{} 
		\State Find the maximal set $\mathcal{P}$ of augmenting paths in $G^t_x$. \label{item:augpath}
		\State Augment along $\mathcal{P}$.  \label{item:augmentation}
		\State Update $\vec{x}$ and $G^t_x$.  \label{item:augmentation2}
		\EndProcedure
	\Procedure{Dual Adjustment:}{}
		\State Let $Z$ be the set of vertices reachable from free left vertices in $G^t_x$.
		\State For all ineligible edges $e_b$ directed from $R\setminus Z$ to $L\cap Z$, $z(e)\leftarrow z(e)+\delta_i$.
		\State For all $u\in L\cap Z$, $y(u)\leftarrow y(u)-\delta_i$.
		\State For all $u\in R\cap Z$, $y(u)\leftarrow y(u)+\delta_i$.
	\EndProcedure
		\EndWhile
	\Procedure{Prepare for next scale:}{}
		\State $\delta_{i+1}\leftarrow \frac{\delta_{i}}{2}$
		\State $y(u)\leftarrow y(u)+2\delta_{i+1}$ for all $u\in L$
	\EndProcedure
		\end{algorithmic}
	 \label{alg:weightedfracmatching}
\end{algorithm}

We now show that the \Cref{alg:weightedfracmatching} preserves \Cref{prop:invariant} throughout. Before this, we start with the following claim.


\begin{observation2}\label{obs:noaugmentingpaths}
After \Cref{item:augmentation} and \Cref{item:augmentation2}, the graph $G^t_x$ doesn't contain any augmenting paths. 
\end{observation2}
\begin{proof}
Suppose $G^t_x$ is the graph before the augmentation, and let $G^t_y$ be the graph after the augmentation. We want to argue that the directed edges of $G^t_y$ are a subset of the directed edges of $G^t_x$. In order to see this, consider an edge $e$, due to the eligibility criterion, either $e_f\in G^t_x$ or $e_b\in G^t_x$ but not both. \\ \\
Without loss of generality, suppose $e_f$ is present in $G^t_x$, and suppose it is augmented along and is saturated by $\vec{y}$. Then, since $G^t_y$ is a residual graph of eligible edges, and the duals of $G^t_x$ and $G^t_y$ are the same, this implies that $G^t_y$ contains neither $e_b$ nor $e_f$. On the other hand, suppose $e_f$ is not saturated by $\vec{y}$, then it appears in $G^t_y$ with capacity at most $\kappa(e)-y(e)\leqslant \kappa(e)-x(e)$, and by the same argument $e_b$ does not appear in $G^t_{y}$. A similar argument applies for $e_b$. Thus, we can conclude that the directed edges of $G^t_y$ are a subset of the edges of $G^t_x$, and therefore, any augmenting path present in the former is present in the latter as well. This contradicts the fact that we found a maximal set of augmenting paths.
\end{proof}

We now show that \textbf{granularity} property holds. 
\begin{claim2}\label{claim:domination}
Throughout \Cref{alg:weightedfracmatching}, \Cref{prop:invariant}\ref{item:gran} is always maintained. 
\end{claim2}
\begin{proof}
We will argue by induction, that for every scale $i=\set{1,\cdots, \log W}$, it holds throughout the scale. First note that it holds at the beginning of each scale, since $\delta_0$ and $W$ are assumed to be powers of $2$. Moreover, $y(u)=W-\eps\cdot W$ for all $u\in L$, and $y(v)=0$ for all $v\in R$, and $z(e)=0$ for all $e\in E$. Consider step \Cref{line:zadj}, suppose for $e=(u,v)$, $z(e)$, $y(u)$ and $y(v)$ were a multiple of $\delta_0$ before this step, then after this step, $z(e)$ is still a multiple of $\delta_0$. This is because $w_i(e)$ is a multiple of $\delta_0$. Similarly, in the dual adjustment procedure, we increment and decrement the duals by $\delta_0$, thus, if they were multiples of $\delta_0$, then they would be multiples of $\delta_0$ even after this step. Finally, when we prepare for the next scale, we make sure that the duals are a multiple of $\delta_1$. We can similarly make such an argument for all $i\geqslant 2$. 
\end{proof}
We now show \textbf{near domination}. 
\begin{claim2}
\Cref{prop:invariant}\ref{item:domin} is maintained throughout the run of \Cref{alg:weightedfracmatching}.
\end{claim2}
\begin{proof}
Observe that \Cref{prop:invariant}\ref{item:domin} holds at the beginning of the $0$th scale. Assume it holds at the beginning of scale $i$. We will show that it holds at the beginning of scale $i+1$ as well. We do so by showing that during scale $i$, each time we change duals, we preserve \textbf{domination}. Consider \Cref{item:zadj}, observe that we modify $z(e)$ in this case if $e_b$ is an eligible edge. This implies that $yz(e_b)\geqslant w(e_b)$. Consequently, after the adjustment to $z(e)$, \Cref{prop:invariant}\ref{item:domin} still holds since after the dual adjusment, $yz(e_b)\geqslant w(e_b)-\delta_i$. \\ \\
Consider now the dual adjustment step, observe that for all edges $e\in E(L\cap Z,R\cap Z)$ and $e\in E(L\setminus Z, R\setminus Z)$ remain eligible after the dual adjustment step since their $yz(e)$ value remains the same. Now, observe there are no eligible edges $e_f\in E(L\cap Z, R\setminus Z)$. This implies that we have $yz(e_f)>  w_i(e_f)-\delta_i$. However, since vertex and edge duals were all multiples of $\delta_i$ (see \Cref{claim:domination}), we can conclude that $yz(e_f)\geqslant w_i(e_f)$. Thus, after dual adjustment step, we have $yz(e_f)\geqslant w_i(e_f)-\delta_i$. Thus, \Cref{prop:invariant}\ref{item:domin} holds after this step. Consider $e_b\in E(R\setminus Z, L\cap Z)$, if this edge is eligible then, after dual adjustment, $yz(e_b)-w_i(e_b)\geqslant -\delta_i$, and domination property still holds. On the other hand, if $e_b$ is ineligible then, we also increment $z(e_b)$, and consequently, $yz(e)$ remains the same, and we still have domination property. \\ \\
Next, consider edges between $R\cap Z$ and $L\setminus Z$, for such edges, since we only increase the duals of $R\cap Z$, and duals of $L\setminus Z$ are unaffected, we still have the domination property. \\ \\
Consider the time when we are preparing for the next scale. In this case, for all vertices $u\in L$, we increment $y(u)$ by $2\delta_{i+1}$. Thus, we have,
\begin{align*}
yz(e)\geqslant w_{i}(e)-\delta_i+2\delta_{i+1}\geqslant w_{i}(e) \geqslant w_{i+1}(e)-\delta_{i+1}
\end{align*}
This proves the claim
\end{proof}
\begin{observation2}
Note that \Cref{prop:invariant}\ref{item:freeduals} holds, since due to property \Cref{obs:noaugmentingpaths}, all free vertices in $L$ are a subset of $L\cap Z$ and all free vertices of $R$ are contained in $R\setminus Z$. Thus, at the beginning of the algorithm, free vertex duals in $R$ are $0$, and they remain $0$ during the rest of the algorithm, since duals of vertices in $R\setminus Z$ are not modified.
\end{observation2}

We now show the complementary slackness property.

\begin{claim2}
Note that \Cref{prop:invariant}\ref{item:slackness} holds throughout the algorithm.
\end{claim2}
\begin{proof}
To see this, observe that $z(e)$ is only incremented when $e_b\in E(R\setminus Z, L\cap Z)$ and $e_b$ is ineligible. Note since $e_b$ is ineligible, it must be the case that $yz(e)-w_i(e)=-\delta_i$. Thus, $e_f$ if it exists, must be eligible, however this would contradict the fact that there can't be eligible forward edges between $R\setminus Z$ and $L\cap Z$. Consequently, $e_f$ doesn't exist, and therefore, we have $x(e)=\kappa(e)$. On the other hand, observe that if $e_b$ with $z(e)>0$ is added to the eligible graph, then it is assured that $z(e)=0$ before $x(e)$ is reduced from $\kappa(e)$ to something lower. This concludes the proof. 
\end{proof}

We now show the tightness property. 

\begin{claim2}
Note that \Cref{prop:invariant}\ref{item:tightness} holds throughout the algorithm. 
\end{claim2}
\begin{proof}
Observe that this holds during the augmentation phase. We now want to show this holds during the dual adjustment phase as well. Note that, as before the edges in $E(L\cap Z, R\cap Z)$ and $E(L\setminus Z, R\setminus Z)$ are unaffected. On the other hand, backward edges in $E(L\cap Z, R\setminus Z)$ will also not have their tighness property affected since $L\cap Z$ is only being decremented. On the other hand, there are no eligible backward edges in $E(R\cap Z, L\setminus Z)$, so the only backward edges are ineligible, which means that $yz(e)=w_{i}(e)-\delta_i$. Thus, after dual adjustment, for such edges, $yz(e)=w_i(e)$, and therefore tightness constraint is satisfied. Finally consider the dual adjustment step that prepares for the next scale, for any backward edge of type $j$, after this step, we have,
\begin{align*}
yz(e)\leqslant w_{i}(e)+2\cdot (\delta_j-\delta_i)+2\delta_{i+1}\leqslant w_{i+1}(e)+2\cdot (\delta_j-\delta_{i+1})
\end{align*}
\end{proof}

Finally, we show the following property of the eligible graph, which will enable us to bound the runtime of the algorithm.

\begin{lemma2}

\end{lemma2}

\subsection{Runtime}

\begin{observation2}
Observe that scale $i$ starts with free duals being $\frac{W-\eps\cdot W}{2^{i+1}}$ and ends with free duals being $\frac{W-\eps\cdot W}{2^{i+1}}$, and each iteration in scale $i$ ends with reducing the dual variables with $\delta_i$, so the total number of iterations in each scale is at most $\frac{1}{\eps}$
\end{observation2}

\begin{observation2}
\Cref{item:zadj} takes time $O(m)$ and is executed once per iteration in the $i$th scale. 
\end{observation2}

\begin{observation2}
\Cref{item:augpath} takes $O(m\cdot \frac{\log n}{\eps})$ time and is executed once per iteration in the $i$th scale.
\end{observation2}

\begin{observation2}
The dual adjustment steps take $O(m)$ time per iteration per scale. 
\end{observation2}

\begin{claim2}
The total runtime of the algorithm is $O(m\cdot \frac{\log n}{\eps}\cdot \log W)$. 
\end{claim2}

==> todo.tex <==
1) table
2) figures?
3) discussion about lemma on fractional matching.
4) proof read
5) intro

